Realistic sensitivity curves for pulsar timing arrays

We construct realistic sensitivity curves for pulsar timing array searches for gravitational waves, incorporating both red and white noise contributions to individual pulsar noise spectra, as well as the effect of fitting to a pulsar timing model. We demonstrate the method on both simulated pulsars and a realistic array consisting of a subset of NANOGrav pulsars used in recent analyses. A comparison between the results presented here and exact sensitivity curves shows agreement to tens of percent. The resulting sensitivity curves can be used to assess the detectability of predicted gravitational-wave signals in the nanohertz frequency band in a fraction of the time that it would take to compute the exact sensitivity curves.

==> manuscript/statistics.tex <==
% !TEX root = pta-sensitivity.tex
\section{Detection statistics, signal-to-noise ratios, and sensitivity curves}
\label{s:detection_statistics}

Ultimately, a detection sensitivity curve should tell us 
how likely it is to detect a particular type of GW signal.
So it should depend not only the properties of the noise 
in the detector, but also on the type of signal that one 
is searching for and the method that one uses to search for it.
So here we extend the formalism of the previous section to 
define sensitivity curves for searches for: 
(i) a deterministic GW signal from a circular binary and 
(ii) an unpolarized, isotropic stochastic GW background.
We begin by writing down expressions for optimal detection
statistics for these two different sources and the 
corresponding expected signal-to-noise ratios (SNRs).
We will see that from these expected SNRs, we can read off
an {\em effective} strain-noise power spectral density, which has
the interpretation of a strain detection sensitivity curve.

\subsection{Matched filtering for a deterministic gravitational 
wave signal}
\label{s:matched}

For a deterministic GW signal, we can use matched 
filtering to construct an optimal detection statistic.
Letting $\mb{Q}_I$ denote the filter function for 
pulsar $I$, we define
%
\be
\hat{\mathcal{S}} 
\equiv \mb{Q}^T\,\mb{r}
=\sum_IQ_{I\alpha}r_{I\alpha} 
\ee
%
where $\mb{Q}\equiv\{\mb{Q}_I\}$ and 
$\mb{r}\equiv\{\mb{r}_I\}$ are the TMM residuals 
defined by \eqref{e:r}.
The filter function is determined by maximizing
the expected signal-to-noise ratio,
$\rho\equiv\mu/\sigma$, of $\hat{\mathcal{S}}$.
The expectation value of $\hat{\mathcal{S}}$ is 
given by
%
\be
\mu \equiv \langle \hat{\mathcal{S}} \rangle 
= \mb{Q}^T{\bf G}^T\mb{h}^{\rm det}
= \sum_I Q_{I\alpha}\,({\bf G}^T_I\mb{h}_I^{\rm det})_\alpha\,,
\ee
%
and its variance is given by
%
\be 
\sigma^2 \equiv
\langle  \hat{\mathcal{S}} ^2 \rangle -
\langle  \hat{\mathcal{S}}\rangle ^2 
= \mb{Q}^T\,\bs{\Sigma}_n\,\mb{Q}
= \sum_I Q_{I\alpha}(\bs{\Sigma}_{nI})_{\alpha\beta}Q_{I\beta}\,,
\ee
%
where 
$\bs{\Sigma}_{nI}\equiv \mb{G}^T_I\mb{C}_{nI}\mb{G}_I$
is the noise covariance matrix for $\mb{r}_I$.
This result for the variance assumes that the only GW 
contribution to the timing residuals is from a deterministic 
GW source, and not from a stochastic GW background.
The presence of a stochastic background would
change the covariance matrix from
$\bs{\Sigma}_{n}$ to $\bs{\Sigma}$, the latter having
GW contributions to both the diagonal and off-diagonal
block matrices, see \eqref{e:Sigma} and \eqref{e:CIJ}.
In what follows, we will assume that the off-diagonal
(cross-correlated) noise is small compared to the 
diagonal (auto-correlated) noise.
But we will replace $\bs{\Sigma}_{nI}$ by 
$\bs{\Sigma}_I\equiv \bs{\Sigma}_{nI}+\bs{\Sigma}_h$, 
thereby allowing for a stochastic GW background 
(self-noise) contribution to the auto-correlated  noise.

Using the above results for the mean and variance
of $\hat{\mathcal{S}}$, 
the square of the expected signal-to-noise ratio is
%
\be 
\rho^2 \equiv
\frac{\mu^2}{\sigma^2} =
\frac{\sum_{I,J} 
Q_{I\alpha}\,({\bf G}^T_I\mb{h}_I^{\rm det})_\alpha\,
Q_{J\beta}\,({\bf G}^T_J\mb{h}_J^{\rm det})_\beta}
{\sum_K Q_{K\mu}(\bs{\Sigma}_{K})_{\mu\nu}Q_{K\nu}}\,,
\ee
%
with the optimal filter given by
%
\be
\begin{aligned}
\frac{\delta\rho^2}{\delta Q_{I\alpha}} = 0 
&\quad\Rightarrow\quad
Q_{I\alpha} = 
(\bs{\Sigma}_{I}^{-1})_{\alpha\beta}
({\bf G}^T_I\mb{h}^{\rm det}_I)_\beta
\quad\Leftrightarrow\quad
\mb{Q}_I = 
\bs{\Sigma}_{I}^{-1}\,
{\bf G}^T_I\,\mb{h}^{\rm det}_I\,.
\end{aligned}
\ee
%
Note that $\mb{Q}_I$  is a noise-weighted version of the 
TMM signal waveform, as expected for matched filtering.
Using this expression, the expected signal-to-noise ratio
becomes
%
\be
\rho^2 
= \sum_I
(\mb{h}_I^{\rm det})^T\,\mb{G}_I\,
\bs{\Sigma}_{I}^{-1}\,
{\bf G}_I^T\mb{h}_I^{\rm det}\,.
\ee
%
This last expression can also be written in terms of the 
Fourier components $\tilde h^{\rm det}_I(f)$ 
of the GW signal defined by 
%
\be
h^{\rm det}_{Ik} 
=\frac{1}{N_I\Delta t_I}\sum_{j=-N_I/2}^{N_I/2-1}
\tilde h_{Ij}^{\rm det}\,e^{i2\pi jk/N_I}
\simeq\int_{-\infty}^\infty 
{\rm d}f\> \tilde h^{\rm det}_{I}(f) e^{i2\pi f t_k}\,.
\label{e:iDFT}
\ee
%
Then
%
\be
\rho^2 \simeq
4 \int_{0}^\infty {\rm d}f
\sum_I 
|\tilde h^{\rm det}_I(f)|^2\,
\mathcal{N}_{I}^{-1}(f)\,,
\label{e:rho2_det}
\ee
%
where
%
\be
\mathcal{N}_{I}^{-1}(f)\equiv
\frac{1}{2 T_I}
\left[\mb{G}_I({\mb G}_I^T \mb{C}_{I}\mb{G}_I)^{-1}\mb{G}_I^T\right]_{kl}
e^{i2\pi f(t_k-t_l)}
\label{e:Ninv_I}
\ee
%
plays the role of 
a (1-sided) inverse-noise power spectral density.
Plots of $\mathcal{N}^{-1}_I(f)$ for white, red, and
red+white noise covariance matrices are shown in 
Figure~\ref{f:Ninvf}.
The large and small downward spikes at 1/yr and 
2/yr correspond to the removal of power in the TMM
residuals due to the timing model fit.
%
\begin{figure}[h!tbp]
\centering
\subfigure[]{\includegraphics[width=0.32\textwidth]{./figures/white_Ninv}}
\subfigure[]{\includegraphics[width=0.32\textwidth]{./figures/red_Ninv}}
\subfigure[]{\includegraphics[width=0.32\textwidth]{./figures/red_white_Ninv}}
\caption{Plots of $\mathcal{N}^{-1}_I(f)$ for different choices
for the covariance matrix $\mb{C}$:
(a) white noise with $\sigma_I=100~{\rm ns}$,
(b) red noise with characteristic amplitude $A=1\times 10^{-15}$
and spectral index $\alpha=-2/3$, 
(c) combined red and white noise given by (a) and (b).
The vertical blue lines correspond to $f=1/T_I= 1/(10~{\rm yr})$.
The horizontal blue lines in panels (a) and (c) correspond
to the inverse of the white noise level, 
$1/(2\sigma_I^2\Delta t_I)$, where $\Delta t_I = 1~{\rm yr}/24$.}
\label{f:Ninvf}
\end{figure}
%

To obtain the above result, we used the
fact that the discrete Fourier transform operation,
defined by the unitary matrix
$U_{jk}\equiv \frac{1}{\sqrt{N}} e^{-i2\pi jk/N}$,
approximately diagonalizes a covariance matrix in 
the limit of a large number of samples $N$.
The values of $\mathcal{N}_{I}^{-1}(f)$, evaluated
at the discrete frequencies $f_j\equiv j/T_I$,
are the (approximate) diagonal elements
of the Hermitian matrix
%
\be
(\bs{\mathcal{N}}_{I}^{-1})_{jj'}
\equiv
\frac{1}{2T_I}
e^{i2\pi jk/N_I}
\left[\mb{G}_I({\mb G}_I^T \mb{C}_{I}\mb{G}_I)^{-1}\mb{G}_I^T\right]_{kl}
e^{-i2\pi j' l/N_I}
\label{e:Ninv_I_jj'}
\ee
%
for $j,j'\in[-N_I/2,N_I/2-1]$. 
(We are assuming here that $N_I$ is even; if $N_I$ is 
odd, then $j,j'\in[-(N_I-1)/2,(N_I-1)/2]$.)
An image plot of the absolute value of these matrix elements 
is given in Figure~\ref{f:Ninv_2d}.
%
\begin{figure}[h!tbp]
\centering
\includegraphics[width=0.5\textwidth]{./figures/Ninv_2d}
\caption{Image plot of the absolute value of the matrix elements
$(\bs{\mathcal{N}}_{I}^{-1})_{jj'}$ defined by 
\eqref{e:Ninv_I_jj'} for the case of red+white noise,
corresponding to panel (c) in Figure~\ref{f:Ninvf}.
Note that this matrix is diagonally dominated, with 
pretty much all of its support on the diagonal $j=j'$.
Here we have plotted only postivite values of $j$ and $j'$.}
\label{f:Ninv_2d}
\end{figure}
%

%We note that since the evolution of the frequency for a SBBH over the lifetime of a PTA is negligible we can take its frequency to be constant, $\omega(t) = \omega_0$, and the amplitude of the polarization tensors can be written 
%
%\be
%\begin{aligned}
%h_+(t;\iota)
%&= h_0 \left(\frac{1+\cos^2\iota}{2}\right)\,e^{i (2\omega_0 t + \varphi)}\,,
%\\
%h_\times(t;\iota)
%&= h_0 \,\cos\iota\,i e^{i (2\omega_0 t + \varphi)}\,.
%\end{aligned}
%\ee
%With this the PTA signal can be written 
%
%\be 
%\begin{aligned}
%h_I = h_0 e^{i (2\omega_0 t + \varphi)}\, \left[\left(\frac{1+\cos^2\iota}{2}\right)\frac{\hat{p}^a_I \hat{p}^b_I \epsilon^{+}_{ab}}{1+\hat p_I \cdot \hat k}  + i \cos\iota\frac{\hat{p}^a_I \hat{p}^b_I \epsilon^{\times}_{ab}}{1+\hat p_I \cdot \hat k}\right]\, ,
%\end{aligned}
%\ee
%
%and we can see that the Fourier amplitude is given by 
%\begin{equation}
%\tilde{h}^{\rm det}_{Ij} = \frac{N_I \Delta t_I}{2} \left[\delta_{-j,A}+\delta_{j,A}\right] h_0 e^{i \varphi}\, \left[\left(\frac{1+\cos^2\iota}{2}\right)\frac{\hat{p}^a_I \hat{p}^b_I \epsilon^{+}_{ab}}{1+\hat p_I \cdot \hat k}  + i \cos\iota\frac{\hat{p}^a_I \hat{p}^b_I \epsilon^{\times}_{ab}}{1+\hat p_I \cdot \hat k}\right],
%\end{equation}
%where $2 \omega_0 = A/(\Delta t_I N_I)$. 

\subsubsection{Simplification for white noise}
\label{s:white_noise_Ninv}

We note that for the case of white noise,
the expression for
$\mathcal{N}_{I}^{-1}(f)$ is particularly simple.
The pre-fit covariance matrix is
%
\be
\mb{C}_{I}=\sigma_I^2\,\bs{\unit}_{N_I\times N_I}\,,
\ee
%
corresponding to the one-sided power spectral 
density 
%
\be
P_{I}(f) = 2\sigma_I^2\,\Delta t_I\,.
\ee
%
Then
%
\be
\bs{\Sigma}_{I} 
\equiv \mb{G}^T_I\mb{C}_{I}\mb{G}_I
= \sigma_I^2\,{\bf G}^T_I
{\bs{\unit}}_{N_I\times N_I}
{\bf G}_I 
= \sigma_I^2\,{\bs{\unit}}_{m_I\times m_I}\,,
\ee
%
where $m_I\equiv N_I-N_{\rm par}$ are the number of
degrees of freedom for TMM residuals.
This implies
%
\be
\mathcal{N}_{I}^{-1}(f)
=\frac{1}{2 T_I}\frac{1}{\sigma_I^2}
(\mb{G}_I\mb{G}_I^T)_{kl}\,e^{i2\pi f(t_k-t_l)}
= \frac{\mathcal{T}_I(f)}{P_{I}(f)}\,,
\label{e:calNn_white_transmission}
\ee
%
or, equivalently,
%
\be
\mathcal{N}_{I}(f) = P_{I}(f)/\mathcal{T}_I(f)\,,
\ee
%
where
%
\be
\mathcal{T}_I(f)
\equiv
\frac{1}{N_I}(\mb{G}_I\mb{G}_I^T)_{kl}\,e^{i2\pi f(t_k-t_l)}
\ee
%
is the {\em transmission function} for pulsar $I$ 
constructed in terms of the $\mb{G}_I$ matrix.
A plot of the G-matrix transmission function 
$\mathcal{T}_I(f)$ corresponding to 
$T_I=10~{\rm yr}$ of data is shown in Figure~\ref{f:TG}.
For the case of white noise, it differs from 
$\mathcal{N}^{-1}_I(f)$ by the overall multiplicative
constant $2\sigma_I^2\Delta t_I$.
%
\begin{figure}[h!tbp]
\centering
\includegraphics[width=0.6\textwidth]{./figures/Tf}
\caption{G-mamtrix transmission functions for 
$T_I=10~{\rm yr}$ of timing data.
The vertical line is at $f=1/T_I$.
As before, the large and small spikes at 1/yr and 2/yr 
correspond to the removal of power in the TMM
residuals due to the timing model fit.}
\label{f:TG}
\end{figure}i
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Detection sensitivity curve for sky and 
inclination-averaged sources}
\label{s:detection_angle_averaging}

To proceed further, we will consider the case of GWs from a single 
binary system averaged over the inclination 
of the source, as well as its sky location.
Using the results from the end of Section~\ref{s:deterministic}
for the angle-averaged values $|\tilde h_I(f)|^2$, we have
%
\be
\langle\rho^2\rangle_{\rm inc,\, sky}
\simeq 4\int_0^\infty {\rm d}f\>
\sum_I \frac{T_I}{2}\frac{4}{5}
\mathcal{R}(f)\tilde S_h(f)\,\mathcal{N}_{I}^{-1}(f)
= 2 T_{\rm obs}\int_0^\infty {\rm d}f\>\frac{S_h(f)}{S_{\rm eff}(f)}\,,
\ee
%
where
%
\be
{S_{\rm eff}(f)}\equiv \left(
\frac{4}{5}\sum_I \frac{T_I}{T_{\rm obs}}\frac{1}{S_I(f)}\right)^{-1}\,,
\qquad
S_I(f) \equiv \frac{\mathcal{N}_I(f)}{\mathcal{R}(f)}\,.
\label{e:Seff_inc,sky}
\ee
%
Here, $S_I(f)$ is the strain noise power spectral
density for pulsar $I$, and $S_{\rm eff}(f)$
is an {\em effective} strain noise power spectral
density for an array of pulsars.
Given how $S_{\rm eff}(f)$ appears in the expression for the
expected signal-to-noise ratio, we will use it as a 
{\em sensitivity curve} for detecting a deterministic 
GW source averaged over the orientation of the source and 
its sky location.
For a monochromatic source, $S_h(f)$ has a very simple 
form given by \eqref{e:Sh(f)_CW}, which implies that
%
\be
\bar\rho
\equiv \sqrt{\langle \rho^2\rangle_{\rm inc,\,sky}}
\simeq h_0\sqrt{\frac{T_{\rm obs}}{S_{\rm eff}(f_0)}}\,.
\ee
%
A plot of $S_{\rm eff}(f)$ for ... is shown in 
Figure~\ref{f:Seff_inc,sky}.
%
\begin{figure}[h!tbp]
\centering
\includegraphics[width=0.4\textwidth]{./figures/placeholder}
\caption{A plot of $S_{\rm eff}(f)$
given by \eqref{e:Seff_inc,sky} for an inclination 
and sky-averaged deterministic source 
for an array of pulsars....}
\label{f:Seff_inc,sky}
\end{figure}
%

\subsubsection{SNR and characteristic amplitude 
sky maps for inclination-averaged sources}
\label{s:skymaps_angle_averaging}

If we average over source inclination but not over sky 
location, using instead $|\tilde h_I(f,\hat k)|^2$, we get
%
\be
\langle\rho^2(\hat k)\rangle_{\rm inc}
\simeq 4\int_0^\infty {\rm d}f\>
\sum_I \frac{T_I}{2}\frac{4}{5}
\mathcal{R}_I(f,\hat k)
\tilde h_0^2(f)\,\mathcal{N}_{I}^{-1}(f)
= 2 T_{\rm obs}\int_0^\infty {\rm d}f\>
\frac{S_h(f)}{S_{\rm eff}(f,\hat k)}\,,
\label{e:rho2(k)}
\ee
%
where
%
\be
S_{\rm eff}(f,\hat k)\equiv \left(
\frac{4}{5}\sum_I \frac{T_I}{T_{\rm obs}}\frac{1}{S_I(f,\hat k)}\right)^{-1}\,,
\qquad
S_I(f,\hat k) \equiv \frac{\mathcal{N}_I(f)}{\mathcal{R}_I(f,\hat k)}\,,
\label{e:Seff_sky}
\ee
%
with $\mathcal{R}_I(f,\hat k)$ given by \eqref{e:calR_I(f,k)}.
These expressions are analogous to \eqref{e:Seff_inc,sky},
but with added dependence on the direction $\hat k$ of the GW.
It turns out that we can factor out the $\hat k$ dependence
on the right-hand side of the above expression for $S_{\rm eff}(f,\hat k)$
if we ignore the frequency-dependent part of the pulsar-term 
contribution to $|R_I^P(f,\hat k)|^2$, as discussed in the 
context of \eqref{e:pulsar-pulsar}.
Making this approximation, 
%
\begin{equation}
S_{\rm eff}(f,\hat k)
\simeq
\left(\frac{12}{5}\sum_I \frac{T_I}{T_{\rm obs}}
\frac{1}{S_I(f)}\,
\left[(F^+_I(\hat k))^2 + (F^\times_I(\hat k))^2\right]
\right)^{-1}\,,
\label{e:Seff(f,k)}
\end{equation}
%
where $F_I^P(\hat k)$ are defined in \eqref{e:FP(k)}.
As before, it is easy to do the integral over frequency
for a monochromatic source, for which $S_h(f)$ is given
by \eqref{e:Sh(f)_CW}.
The result is
%
\be
\rho(\hat n)\equiv 
\sqrt{\langle \rho^2(\hat k)\rangle_{\rm inc}}
\simeq h_0 \sqrt{\frac{T_{\rm obs}}{S_{\rm eff}(f_0,\hat k)}}\,,
\label{e:rho(n)}
\ee
%
where the direction $\hat n$ of the source on the sky 
is opposite the direction of GW propagation, $\hat n=-\hat k$.
A plot of $\rho(\hat n)$ for a pair of $10^9$~solar-mass 
black holes at a luminosity distance of 100~Mpc, 
emitting monochromatic GWs at the frequency $f_0 = 8~{\rm nHz}$
is shown in Figure~\ref{f:rho(n)}.
%
\begin{figure}[h!tbp]
\centering
\includegraphics[width=0.7\textwidth]{./figures/SNR_skymap}
\caption{A sky-map of $\rho(\hat n)$ for a 
a circular binary consisting of a pair of 
$10^9$~solar-mass black holes at a luminosity 
distance of 100~Mpc.
The PTA consists of...}
\label{f:rho(n)}
\end{figure}

Finally, it is a simple matter to recast the form of the 
sky map so that we solve \eqref{e:rho(n)} 
for the strain amplitude $h_0$ of a monochromatic binary, 
cf.~\eqref{e:h0}, that would 
produce a particular value of the signal-to-noise ratio 
$\rho$:
%
\be
h_0(\hat n)
= {\rho}\sqrt{\frac{S_{\rm eff}(f_0,\hat k)}{T_{\rm obs}}}\,.
\ee
%
A sky map of $h_0(\hat n)$ is shown in 
Figure~\ref{f:Agw_map} for $\rho=2$.
%
\begin{figure}[h!tbp]
\centering
\includegraphics[width=0.7\textwidth]{./figures/Agw_skymap}
\caption{The sky map $h_0(\hat n)$ for a monochromatic 
binary with $f_0 = 8~{\rm nHz}$ and $\rho=2$.
Here we've considered an array of pulsars ....}
\label{f:Agw_map}
\end{figure}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimal statistic for a gravitational wave background}
\label{s:optimal_GWB}

The derivation of the optimal cross-correlation statistic 
for a stochastic GW background is similar to that 
presented above for a deterministic GW, expect that we
work with data from pairs of pulsars.
Starting with a single distinct pair, labeled by $I$ 
and $J$, we define
\be
\hat{\mathcal{S}}_{IJ} \equiv  
\mb{r}_I^T \mb{Q}\, \mb{r}_J
=r_{I\alpha}Q_{\alpha\beta}\,r_{J\beta}\,,
\ee
%
where $\mb{r}_I$ and $\mb{r}_J$ are the TMM residuals 
for pulsars $I$ and $J$ 
(assuming that we've already fit for all deterministic
GW sources), and $\mb{Q}$ is an $m_{IJ}\times m_{IJ}$ matrix,
where $m_{IJ}\equiv N_I-N_{\rm par}\>(= N_J-N_{\rm par})$,
with the number of TOAs for the two pulsars equal to
one another, $N_I=N_J$.
As before, we determine the filter function $\mb{Q}$
by maximizing the signal-to-noise ratio of $\hat{\mathcal{S}}_{IJ}$.
Similar derivations appear in the literature (TO-DO: ADD REFS).
The final result for the optimal filter 
%
\be
\mb{Q} \propto \,\bs{\Sigma}_I^{-1}
\bs{\Sigma}_{IJ}\bs{\Sigma}_J^{-1}\,,
\ee
%
where 
%
\begin{align}
&\bs{\Sigma}_I
\equiv \mb{G}_I^T(\mb{C}_{I} + \mb{C}_h)\mb{G}_I\,,
\qquad{\rm etc.}\,,
\\
&\bs{\Sigma}_{IJ}
\equiv \chi_{IJ}\,\mb{G}_I^T \mb{C}_h \mb{G}_J\,.
\end{align}
%
The squared expected signal-to-noise ratio for this
optimal choice of the filter $\mb{Q}$ is
%
\begin{equation}
\rho_{IJ}^2 = 
{\rm Tr}\left[\bs{\Sigma}_{JI}\,\bs{\Sigma}_I^{-1}
\bs{\Sigma}_{IJ}\bs{\Sigma}_J^{-1}\right]\,.
\end{equation}
%
The above calculation assumes that we are in the 
weak-signal limit where the cross-correlation terms
are assumed to be negligible compared to auto-correlation
terms.

We can then combine the signal-to-noise ratios for 
each distinct pair in quadrature since, 
in the weak-signal limit, 
there is negligible correlation between these estimators: 
%
\begin{equation}
\rho^2 \simeq 
\sum_{I}\sum_{J>I} \rho_{IJ}^2.
\end{equation}
%
As we saw for deterministic GWs, it is useful to write
the above expression for the expected squared signal-to-noise
ratio in the frequency domain.
Proceeding as we did there, we find
%
\be
\rho^2
\simeq \sum_I \sum_{J>I}
2 T_{IJ}\chi_{IJ}^2
\int_{0}^\infty{\rm d}f\>
S^2_h(f) \mathcal{R}^2(f)
\mathcal{N}^{-1}_I(f)
\mathcal{N}^{-1}_J(f)\,,
\ee
%
where $P_h(f) = \mathcal{R}(f)S_h(f)$, and
where $\mathcal{N}_I^{-1}(f)$ is defined by
\eqref{e:Ninv_I}.
This suggests defining the 
following {\em effective} noise power 
spectral density for the whole network
%
\be
S_{\rm eff}(f)
=
\left(\sum_I\sum_{J>I} 
\frac{T_{IJ}}{T_{\rm obs}}
\frac{\chi^2_{IJ}}{S_I(f)S_J(f)}
\right)^{-1/2}
\ee
%
which includes contributions from the Hellings and 
Downs factors $\chi_{IJ}$ and the individual pulsar
sensitivity curves $S_I(f)\equiv \mathcal{N}_I(f)/\mathcal{R}(f)$.
Note that $S_{\rm eff}(f)$ has dimensions of strain${}^2$/Hz,
and that
%
\be
\rho^2\simeq 
2T_{\rm obs}\int_0^\infty{\rm d}f\>
\frac{S_h^2(f)}{S_{\rm eff}^2(f)}
\ee
%
in terms of $S_{\rm eff}(f)$.


